Volume uncertainty assessment method of asteroid models from disk-integrated visual photometry

The need for more accurate asteroid models is perhaps secondary to the need to measure their quality. The uncertainties of models' parameters propagate to quantities like volume or density -- the most important and informative properties of asteroids -- affecting conclusions about their physical nature. Our knowledge on shapes and spins of small solar system bodies comes mostly from visual, disk-integrated photometry. In this work we present a method for asteroid model uncertainty assessment based on visual photometry (lightcurves and sparse-in-time absolute measurements) allowing the determination of realistic volume uncertainty, as well as spin axis orientation, rotational period and local surface features. The sensitivity analysis is conducted by creating clones of the nominal model and accepting the ones that fit the observations within a confidence level. The uncertainties of model parameters are extracted from the extreme values found in the accepted clone population. Creation of such population of clones enables the conversion of a deterministic asteroid model into stochastic one, and can be utilized to create observation predictions with error bars. The method was used to assess the uncertainties of fictitious test models and real targets, i.e. (21) Lutetia, (89) Julia, (243) Ida, (433) Eros and (162173) Ryugu. We conclude that volumes, and subsequently, densities of asteroids derived from lightcurve-based models likely have vastly understated uncertainties, the biggest source of which is the inability to establish the extent of the model along its spin axis.

==> img/tab_juno_obs.tex <==
\begin{table*}
	\caption{Details of the lightcurve data used for (3) Juno modelling and
		uncertainty assessment. N$_{lc}$ -- number of lightcurves per
		apparition, $\alpha$
 -- phase angle, $\lambda$ -- ecliptic longitude, $\beta$ -- ecliptic latitude.}
\label{tab:juno_lc}
\begin{tabular}{ccccccc}
\hline
\hline
  Apparition & Year & N$_{lc}$ & $\alpha$ $[^{\circ}]$ & $\lambda$ $[^{\circ}]$
& $\beta$ $[^{\circ}]$ & reference\\
\hline
  1  & 1954 &  3  &     8-15    &  134  & -8   & \cite{groeneveld54b}\\
  2  & 1958 &  1  &     24      &  94   & -13  & \cite{gehrels62}\\
  3  & 1970 &  1  &     19      &  38   & -9   & \cite{Birch1989}\\
  4  & 1973 &  2  &     7       &  256  & 13   & \cite{Birch1989}\\
  5  & 1979 &  5  &     17-30   &  79-102  & 12   & \cite{Millis1981}\\
    &  &    &        &    &                       & \cite{Harris1989a}\\
  6  & 1980 &  5  &      5      &  121     & -10  & \cite{Schroll1981}\\
  7  & 1983 &  2  &      8      &  31      & -9   & \cite{dimartino1987b}\\
  8  & 1985 &  8  &    3-10     &  184-189 & 4    & \cite{Birch1989}\\
  9  & 1985 &  1  &    22       &  147     & -5   & \cite{Viikinkoski2015}\\
\hline
\end{tabular}
\end{table*}






==> img/tab_metis_obs.tex <==
\begin{table*}
	\caption{Details of the lightcurve data used for (9) Metis modelling and
		uncertainty assessment. N$_{lc}$ -- number of lightcurves per
		apparition,   $\alpha$
 -- phase angle, $\lambda$ -- ecliptic longitude, $\beta$ -- ecliptic latitude.}
\label{tab:metis_lc}
\begin{tabular}{ccccccc}
\hline
\hline
  Apparition & Year & N$_{lc}$ & $\alpha$ $[^{\circ}]$ & $\lambda$ $[^{\circ}]$ & $\beta$ $[^{\circ}]$ & reference\\
\hline
  1  & 1949 &  1  &     2.5    &  41.1  & -5.0  & \cite{groeneveld54a}\\
  2  & 1954 &  4  &  3.0 -- 9.4& 97.4  &  5.6  & \cite{groeneveld54b}\\
  3  & 1958 &  1  &     5.1    & 153.1  &  9.6  & \cite{gehrels62}\\
  4  & 1962 &  2  &  3.5--5.1    & 195.0  &  7.8  & \cite{chang62}\\
  5  & 1964 &  1  &    16.4    &  94.5  &  1.5  & \cite{yang65}\\
  6  & 1974 &  1  &     8.5    & 294.0  & -5.3  & \cite{zappala79}\\
  7  & 1978 &  3  & 4.3 -- 13.2& 320.0  & -9.0  & \cite{schober79}\\
  8  & 1979 &  3  &23.0 -- 24.2& 140.2  &  6.0  & \cite{harris89}\\
  9  & 1982/1983 & 3 & 8.5 -- 24.0 & 32.0 & -1.1 & \cite{dimartino84},\\
     & & & & & & \cite{weiden87}\\
 10  & 1984 &  8  & 3.5 -- 13.5& 178.0 & 8.9 & \cite{zeigler85},\\
     & & & & & & \cite{dimartino87},\\
     & & & & & & \cite{weiden87}\\
 11  & 1985 &  2  & 4.4 -- 5.2 & 286.0  & -4.8  & \cite{weiden87}\\
 12  & 1986 &  3  & 2.2 -- 3.8 &  67.0 & -0.8 & \cite{melillo87}\\
 13  & 1988 &  2  & 2.3 -- 2.8 & 214.0  &  5.0  & \cite{weiden90}\\
\hline
\end{tabular}
\end{table*}

